Anonymizing Sensor Data on the Edge: A Representation Learning and Transformation Approach

The abundance of data collected by sensors in Internet of Things (IoT) devices, and the success of deep neural networks in uncovering hidden patterns in time series data have led to mounting privacy concerns. This is because private and sensitive information can be potentially learned from sensor data by applications that have access to this data. In this paper, we aim to examine the tradeoff between utility and privacy loss by learning low-dimensional representations that are useful for data obfuscation. We propose deterministic and probabilistic transformations in the latent space of a variational autoencoder to synthesize time series data such that intrusive inferences are prevented while desired inferences can still be made with sufficient accuracy. In the deterministic case, we use a linear transformation to move the representation of input data in the latent space such that the reconstructed data is likely to have the same public attribute but a different private attribute than the original input data. In the probabilistic case, we apply the linear transformation to the latent representation of input data with some probability. We compare our technique with autoencoder-based anonymization techniques and additionally show that it can anonymize data in real time on resource-constrained edge devices.

==> acmart-preload-hook.tex <==
\PassOptionsToPackage{monochrome}{xcolor}

==> dataset.tex <==
\section{Datasets}
We use two HAR datasets. These datasets include, the MotionSense and the MobiAct datasets.
\subsection{MotionSense dataset}
MotionSense~\cite{malekzadeh19} HAR timeseries dataset is
collected from accelerometer and gyroscope sensors. This dataset is collected from iPhone~6s using the Sensing Kit framework~\cite{katevas2016sensingkit}. This dataset has 24 subjects (14 males and 10 females), 
each doing 15 trials that include 6 different activities. These activities include moving downstairs, moving upstairs, walking, jogging, sitting, and standing. The subjects' age, height, and weight cover a wide range of values. The dataset is collected at 50 Hz sample rate and each sample contains 12 features including attitude (roll, pitch, yaw), 
gravity, rotation rate, and user acceleration in three dimensions, $x$, $y$, and~$z$.

% As described in~\cite{malekzadeh19}, the smartphone is placed inside the pocket of the subjects wearing slim fit pants.
% This helps to obtain the most distinctive features about the subjects' movements and inhibits sudden phone movements (e.g., jolting effects)
% which could otherwise happen when the subject is running.

We use windows of $128$ samples, each corresponding to time series data sampled over $2.56$ seconds. These windows are moved with strides of 10 samples. This is the same configuration used in the implementation of~\cite{malekzadeh19}. 
This is essential to keep the evaluation results comparable. 
From the $6$ different activities mentioned earlier, standing and sitting have quite similar features. Since the phone is placed in the pocket of a subject's pant, 
the only distinction between standing and sitting activities
is the position of the smart phone in the pocket of the users which differs
from vertical to horizontal. 
Hence, we combine both of these activity labels into one activity label.
We use trials $11$, $12$, $13$, $14$, $15$, and $16$ from this dataset to form our test set. We treat each of these $4$ activity classes as a utility class, $u$ and refer to each gender group $0$ and $1$ in the data as the intrusive class, $i$.

\subsection{MobiAct dataset}
MobiAct dataset is comprised of sensor readings in smart phones were the participants and study subjects perform a range of falls alongside a wide range of activities~\cite{vavoulas2016mobiact}. This dataset is larger compared to the MotionSense dataset both in the number of activities and the number of participants. There are $66$ participants in the MobiAct dataset performing $12$ daily lives activities such as running, jogging, going up and down the stairs and many more. Along side these $12$ activities, the subjects perform $4$ different types of falls. From the $66$ participants, we use only $37$ in order to create a balanced dataset with roughly the same number of female to male participants. There are $17$ females, referred to as gender $1$, and $20$ males, gender $0$. Furthermore, we use ternary weight categorical data anonymization to showcase the ability of our anonymization technique. We label subjects that weigh less than or equal to $70$ Kgs as $0$, and individuals weighing between $70$ to no more than $90$ Kgs as $1$. Finally, those individuals that weigh upwards of $90$ Kgs are assigned label $2$.

From the large list of the MobiAct activites, we select four were all of the participants have representative data and sensor readings. These activities include Walking, Standing, Jogging, and Stairs Up (WAL, STD, JOG, and STU according to the activity labels in the dataset).
% One important difference in the MobiAct dataset evaluation is that instead of using the magnitude of each sensor reading, which resulted in poor activity and gender identification accuracies, we used the raw sensor readings from all the three axes ($x$, $y$, and $z$). Now by using both the Gyroscope and Accelerometer sensor readings, we would have 6 data attributes per each data entry, this fact would in turn require more deep neural network models to cope with the now less parsimonious activity and gender detection models. Also, more layers are required in the encoder and decoder portions of the VAE to have the same performance compared to the MotionSense dataset. The embeddings are also built according to the algorithm mentioned in the MotionSense dataset time series to embedding conversion, where windows of $128$ samples are used with strides of $10$.
As not every the activities is performed for more than one trial, we use subject based test and train data partitioning. We divide the dataset between train and test sets. We use $80\%$ for training set and $20\%$ for the test set

==> discussion.tex <==
\section{Discussion}
\label{discussion}

Our evaluation results show the enhancement effect of the proposed modifications to our model-free anonymization technique~\cite{hajihass2020latent}. All in all, the technique is proposed and tested on categorical data anonymization. This is mostly the case in the IoT sensor data analytics. However, study of real valued data predictions is important as well. We notify the reader that the current model-free anonymization technique, is proposed for categorical data anonymization. This is due to the fact that the latent representation manipulation technique relies on different class labels in the data.

Moreover, although it would not be computationally sound to send the probabilistic decoders computation to a GPU-based cloud server. It can be studied based on power consumption and energy saving reasons. Although, the probabilistic decoder execution time is comparatively shorter than the probabilistic encoder, it might still be worth while to study the energy saving effect of edge and server cooperative anonymization.

Apart from these two discussion points, the proposed modified model-free anonymization technique proves to firstly be more performant in data anonymization. And, secondly, to be less susceptible to the re-identification model. Moreover, the proposal of the utility-based specialized VAE models proves to be benefitial in real-time edge anonymization.
